Parameterized Ekman boundary layers on the tilted $f$-plane

Rotating convection is considered on the tilted $f$-plane where gravity and rotation are not aligned. For sufficiently large rotation rates, $\Omega$, the Taylor-Proudman effect results in the gyroscopic alignment of anisotropic columnar structures with the rotation axis giving rise to rapidly varying radial length scales that vanishes as $\Omega^{-1/3}$ for $\Omega\rightarrow\infty$. Compounding this phenomenon is the existence of viscous (Ekman) layers adjacent to the impenetrable bounding surfaces that diminish in scale as $\Omega^{-1/2}$. In this investigation, these constraints are relaxed upon utilizing a non-orthogonal coordinate representation of the fluid equations where the upright coordinate aligns with rotation axis. This exposes the problem to asymptotic perturbation methods that permit: (i) relaxation of the constraints of gyroscopic alignment; (ii) the filtering of Ekman layers through the uncovering of parameterized velocity pumping boundary conditions; and (iii) the development of reduced quasi-geostrophic systems valid in the limit $\Omega\rightarrow\infty$. Linear stability investigations reveal excellent quantitative agreement between results from parameterized or unapproximated mechanical boundary conditions. For no-slip boundaries, it is demonstrated that the associated Ekman pumping dramatically alters convective onset through an enhanced destabilization of large spatial scales. The range of unstable modes at a fixed thermal forcing is thus significantly extended with a direct dependence on $\Omega$. This holds true even for geophysical and astrophysical regimes characterized by extreme values of the non-dimensional Ekman number $E$. The nonlinear regime is explored via the global heat and momentum transport of single-mode solutions to the quasi-geostrophic systems which indicate $\mathcal{O}(1)$ changes irrespective of the smallness of $E$.

==> preamble.tex <==
\textwidth 6in
\textheight 9in
\topmargin -0.5in
\oddsidemargin 0.25in

%\pagestyle{myheadings}
%\markright{Technical Note \# 0005 \copyright\ April 1996 Julien}

\catcode`\@=11      %amh allows redefinition of latex2e definitions
\newenvironment{acknowledgments}{\par\vskip 10pt plus 1pt minus 1pt}{\par}
\newcommand{\rmn}[1] {{\rm #1}}
\renewcommand{\section}{\@startsection {section}{1}{\z@}%
                                   {-1.25ex \@plus -1ex \@minus -.2ex}%
                                   {0.5ex \@plus.2ex}%
                                   {\reset@font\normalsize\bfseries}}
\renewcommand{\subsection}{\@startsection{subsection}{2}{\z@}%
                                     {-1.25ex\@plus -1ex \@minus -.2ex}%
                                     {0.5ex \@plus .2ex}%
                                     {\reset@font\normalsize\bfseries}}

\def\@biblabel#1{} % remove label from bibliography listing
\def\thebibliography#1{%
\def\bibls{\kern.065em}% for letterspacing; normally .15em
\par\vskip 1.0ex plus 1.0ex minus 0.2ex
\centerline{\hspace{1.625in}\hrulefill\hspace{1.625in}}
\nobreak
 \list{}{\labelwidth\z@ \leftmargin 2em \itemindent -2em \itemsep 1pt}
 \reset@font\small \parindent\z@
 \parskip\z@ plus .1pt\relax
 \def\newblock{\hskip .11em plus .33em minus .07em}
 \sloppy\clubpenalty4000\widowpenalty4000
 \sfcode`\.=1000\relax}
\let\endthebibliography=\endlist

\catcode`\@=12      %amh @ back to normal use

\usepackage{graphics}
\usepackage{subequation}
%---------------------------------------------------------- Definitions.
\newcommand{\Rey}{\mbox{\it Re}}
\newcommand{\Pe}{\mbox{\it Pe}}
\newcommand{\Pran}{\ensuremath{\sigma}}
\newcommand{\Ra}{\mbox{\it Ra}}
\newcommand{\Ta}{\mbox{\it Ta}}
\newcommand{\Ro}{\mbox{\it Ro}}
\newcommand{\Nu}{\mbox{\it Nu}}
\newcommand{\Fr}{\mbox{\it Fr}}
\newcommand{\half}{{\textstyle{1\over 2}}}


\newcommand{\ie}{\mbox{\it i.e.}}
\newcommand{\eg}{\mbox{\it e.g.}}
\newcommand{\etc}{\mbox{\it etc.}}
\newcommand{\etal}{\mbox{\it et al.}}

\def\begineq{\begin{equation}}
\def\endeq{\end{equation}}

\def\begineqn{\begin{equation*}}
\def\endeqn{\end{equation*}}

\def\beginar{\begin{eqnarray}}
\def\endar{\end{eqnarray}}
\def\beginarn{\begin{eqnarray*}}
\def\endarn{\end{eqnarray*}}

\def\lb{\left ( }
\def\rb{\right ) }
\def\lsq{\left [ }
\def\rsq{\right ] }
\def\efma{\frac{1}{\epsilon}}
\def\efmb{\frac{\epsilon^2}}
\def\efmc{\frac{\epsilon^3}}
\def\efmd{\frac{\epsilon^4}}
\def\ema{\epsilon^{-1}}
\def\emb{\epsilon^{-2}}
\def\emc{\epsilon^{-3}}
\def\emd{\epsilon^{-4}}
\def\eme{\epsilon^{-\frac{1}{2}}}
\def\ep{\epsilon}
\def\epb{\epsilon^{2}}
\def\epc{\epsilon^{3}}
\def\eph{\epsilon^{\frac{1}{2}}}

\def\srhoz{{\overline\rho}(z)}
\def\rhoz{{\overline\rho}(Z)}
\def\drhoz{\partial_Z{\overline\rho}(Z)}
\def\sdrhoz{\partial_z{\overline\rho}(z)}
\def\src{{\cal S}}

\def\ub{{\bf u}}
\def\vb{{\bf v}}
\def\vkb{{\bf \widehat v}}
\def\dt{{\partial_T}}
\def\dx{{\partial_X}}
\def\dy{{\partial_Y}}
\def\dyy{{\partial_{YY}}}
\def\dsx{{\partial_x}}
\def\dsy{{\partial_y}}
\def\dsyy{{\partial_{yy}}}
\def\dsz{{\partial_z}}
\def\dszz{{\partial_{zz}}}
\def\dszzz{{\partial_{zzz}}}
\def\dz{{\partial_Z}}
\def\dzz{{\partial_{ZZ}}}
\def\dzzz{{\partial_{ZZZ}}}
\def\hz{{\bf\widehat z}}
\def\hy{{\bf\widehat y}}
\def\hx{{\bf\widehat x}}
\def\ldb{{\langle\hspace{-0.5em}\langle}}
\def\rdb{{\rangle\hspace{-0.5em}\rangle}}
\def\om{\mbox{\boldmath $\widehat\eta$}}
\def\omc{\mbox{\boldmath $\widehat\xi$}}
\def\zt{\mbox{\boldmath $\widehat\zeta$}}
\def\omb{\mbox{\boldmath $\omega$}}
\def\tnb{\widetilde\nabla}
\def\hnb{\widehat\nabla}
\def\tdt{{\widetilde\nabla}^2}
\def\md{D^\perp_t}

\newbox\grsign \setbox\grsign=\hbox{$>$} \newdimen\grdimen
\grdimen=\ht\grsign
\newbox\simlessbox \newbox\simgreatbox
\setbox\simgreatbox=\hbox{\raise.5ex\hbox{$>$}\llap
     {\lower.5ex\hbox{$\sim$}}}\ht1=\grdimen\dp1=0pt
\setbox\simlessbox=\hbox{\raise.5ex\hbox{$<$}\llap
     {\lower.5ex\hbox{$\sim$}}}\ht2=\grdimen\dp2=0pt
\def\simgreat{\mathrel{\copy\simgreatbox}}
\def\simless{\mathrel{\copy\simlessbox}}

\newfam\msyfam
\def\msy@{\hexnumber\msyfam}

